On Ellipsoidal Collapse and Primordial Black-Hole Formation

We reinvestigate gravitational ellipsoidal collapse with special focus on its impact on primordial black-hole formation. For a generic model we demonstrate that the abundance and energy density of the produced primordial black holes will be significantly decreased when the non-sphericity of the overdensities is taken into account.

==> Constraints.tex <==
The process of gravitational collapse is of utmost importance to our understanding of the Universe. From the formation of galaxies \cite{Blumenthal:1984bp,Kauffmann:1993gv}, clusters of galaxies \cite{White:1977jf,Davis:1985rj}, haloes \cite{Navarro:1995iw,Navarro:1996gj,Moore:1999nt,Bullock:1999he,Cooray:2002dia} (for a recent review see \cite{Frenk:2012ph}) or even to the possible formation of primordial black holes \cite{Carr:1974nx, Carr:2009jm, Khlopov:2008qy}, the nature of the collapse is crucial in determining characteristics like abundance, mass or shape.

In many cases, both for its calculational simplicity as well as being a reasonable first approximation, spherical symmetry has been an integral assumption to investigate gravitational collapse processes \cite{Misner:1964je, Penrose:1964wq, Penrose:1969pc}. Although in most cases initial non-sphericity is either small or eventually leads to (approximately) spherical objects, its effect might nevertheless be consequential. For instance, estimates of the abundance of small galactic haloes receive considerable corrections \cite{Sheth:1999su}, %the collapse time decreases significantly \cite{...}, 
the formation of space-time singularities might be very different \cite{Shapiro:1991zza}, or, the precise geometric way in which collapse proceeds may lead to major intermediate deformations \cite{1965ApJ...142.1431L, Thorne:1972ji}.

%Though non-sphericity may lead to small corrections in most observables, it might largely effect others. An example is the abundance of massive objects, which depends (approximately) exponentially on their formation threshold, and deviations in this of a few percent might lead to a change of the former by an order of magnitude.}

The space of all possible shapes a collapsing overdensitiy might have is enormously large. Hence, one needs to focus on the most relevant structures. One of the simplest and most studied, deviating from spherical symmetry, is an ellipsoidal one, also because it gives a fairly good approximation to objects of many shapes. This has been and still is the focus of a vast amount of literature (\cf~\cite{1993A&A...280..351B, Eisenstein:1994ni, Bond:1993we, Monaco:1994ed, Monaco:1997cq, Sheth:1999su, Sheth:2001dp, Ohta:2004mx}), including the seminal work of Sheth, Mo and Tormen \cite{Sheth:1999su} who obtained a fitting formula for the mentioned collapse threshold which they found to be supported by numerical evidence. More recent evidence for the improvement of fits with an ellipsoidal collapse model can be found for instance in \cite{Robertson:2008jr, Angrick:2010qg}.

While most of the quoted references on ellipsoidal collapse deal with the formation of dark-matter haloes, the investigation of how the shape distribution of initial overdensities may affect the formation of primordial black holes is relatively modest. In \cite{Baumgarte:2015aza} the authors studied tri-axial collapse of black holes and critical collapse in a way which is relevant also for primordial black-hole formation, and in \cite{Clough:2016jmh} a non-spherical critical collapse was considered. The authors of \cite{Khlopov:1980mg, 1981SvA....25..406P, 1982SvA....26..391P} discussed effects of non-spherical geometry in the formation of primordial black holes if it occurred during an intermediate phase of matter domination due to a superheavy unified field theory particle in the very early universe. However, to the best of our knowledge, there has not been a thorough investigation of the effect of the abundance, or, the energy density of primordial back holes when lifting the spherical assumption on the overdensities in a general situation.

This is what we are going to study here. Specifically, we shall first argue that the ellipsoidal collapse threshold in the case of primordial black holes should be similar to that found in halo formation with only small deviation to the exact fitting constants. As we shall argue, the details of the radiation medium will essentially be contained in the spherical collapse threshold which has been obtained in the case for primordial black holes through detailed numerical studies \cite{Musco:2004ak, Musco:2008hv, Musco:2012au}. We will then investigate the influence of non-spherical effects on the final mass-density spectrum for a generic model of primordial black-hole formation.

To start, the ellipsoidal collapse threshold obtained by Sheth, Mo \& Tormen (\cf~Eq.~(3) of Ref.~\cite{Sheth:1999su}) for the case of halo collapse can be expressed via
\begin{align}
	\frac{ \delta_{\rm ec} }{ \delta_{\crm} }
		&\simeq
								1
								+
								\kappa\mspace{-1mu}
								\left(
									5\.e^{2}\.
									\frac{ \delta_{\rm ec} }{ \delta_{\crm}^{2} }
								\right)^{\!\!\gamma}
		=
								1
								+
								\kappa\mspace{-1mu}
								\left(
									\frac{ \sigma^{2} }{ \delta_{\crm}^{2} }
								\right)^{\!\!\gamma}
								,
								\label{eq:Sheth-Mo-Tormen}
\end{align}
with the threshold value for spherical collapse $\delta_{\crm}$, the ellipticity $e$, and the hight of the density power spectrum at the given scale $\sigma^{2}$. The parameter values for $\kappa$ and $\gamma$ were found to be $0.47$ and $0.62$, respectively. The final equality holds after inserting the most-probable (mp) value for the ellipticity, $e_{\rm mp} = \left(\sigma/\delta\right)/\sqrt{5}$. Actually, this is not entirely correct as the average value $\left< e \right> = 9 / \sqrt{10\pi\,}\.( \sigma / \delta ) \neq e_{\rm mp}$, as was pointed out in \cite{Angrick:2010qg}. There they found another set of values for $\kappa=0.6536$ and $\gamma=0.6387$ \cite{Angrick:2010qg}.

The above result \eqref{eq:Sheth-Mo-Tormen} has been derived and numerically confirmed for a very limited class of cosmologies only, mostly relevant to structure formation. This in particular does not include the case of ellipsoidal collapse in radiation domination, which is the most important one for primordial black-hole formation\cite{Carr:2009jm}. Below, for a Gaussian-distributed density-perturbation spectrum, we shall justify why the functional form of Eq.~\eqref{eq:Sheth-Mo-Tormen} is relevant also for the case of primordial black-hole formation. In fact, by giving an approximate physical argument in which both the derivation and the approximations made are dependent only upon the geometry of the collapse process, we suggest that the form Eq.~\eqref{eq:Sheth-Mo-Tormen} should indeed hold for ellipsoidal gravitational collapses in arbitrary environments.

==> CoordinatesEq.tex <==
Metrics and coordinates for the ellipsoid with ellipticity $e$ and prolateness $p = 0$:

\begin{eqnarray}
	ds^2 &=& -c^2dt^2 + a^2(t)\left[d\chi^2 + \sin^2\chi d\Omega^2 - e^2\left(\cos\theta d\chi + \sin\chi\sin\theta d\theta\right)^2\right]\nonumber\\
	ds^2 &=& -c^2dt^2 + a^2(t)\left[\frac{dr^2}{1-Kr^2} + r^2 d\Omega^2 - e^2\left(\frac{\cos\theta dr}{\sqrt{1-Kr^2}} + r\sin\theta d\theta\right)^2\right]\nonumber
\end{eqnarray}
where $K = 1$ and $r = \sin\chi$.

This means that the metric non-zero elements are:
\begin{eqnarray}
	g_{tt} = -c^2, \qquad g_{rr} = \frac{a^2}{1-Kr^2}(1-e^2\cos^2\theta), \qquad g_{\phi\phi} = a^2r^2\sin^2\theta,\nonumber\\
	g_{\theta\theta} = a^2r^2(1-e^2\sin^2\theta), \qquad g_{r\theta}=g_{\theta r}=-\frac{e^2r\sin\theta\cos\theta}{\sqrt{1-Kr^2}}a^2,
\end{eqnarray}
and the non-zero elements of the inverse metric are:
\begin{eqnarray}
	g^{tt} = -\frac{1}{c^2}, \qquad g^{rr} = \frac{\left(1 -Kr^2\right)}{a^2\left(1-e^2\right)}(1-e^2\sin^2\theta), \qquad g^{\phi\phi} = \frac{1}{a^2r^2\sin^2\theta},\nonumber\\
	g^{\theta\theta} = \frac{1-e^2\cos^2\theta}{a^2r^2(1-e^2)}, \qquad g^{r\theta}=g^{\theta r}=\frac{e^2\sin\theta\cos\theta\sqrt{1-Kr^2}}{ra^2\left(1-e^2\right)}.
\end{eqnarray}

From this we can obtain the non-zero Christoffel symbols:
\begin{eqnarray}
\Gamma^t_{rr} = {\dot{a}a\left(1 - e^2\cos^2\theta\right)}{c^2\left(1-Kr^2\right)}, \qquad\Gamma^t_{\theta\theta} = {\dot{a}a}{c^2}r^2\left(1 - e^2\sin^2\theta\right), \nonumber\\
\Gamma^{t}_{r\theta}=\Gamma^{t}_{r\theta} = -\frac{\dot{a}a e^2r\sin\theta\cos\theta}{c^2\sqrt{1-Kr^2}},  \qquad \Gamma^{r}_{rr} = \frac{Kr}{1-Kr^2} -\frac{e^4\sin^2\theta\cos^2\theta}{r\left(1-e^2\right)}\left(1 + \frac{1}{\sqrt{1-Kr^2}}\right),\nonumber \\
 \Gamma^{r}_{tr}=\Gamma^{r}_{rt} = \frac{\dot{a}}{a}, \qquad \Gamma^{r}_{r\theta}=\Gamma^{r}_{\theta r} = \frac{e^2\sin\theta\cos\theta}{1-e^2}\left(1-e^2\sin^2\theta\right)\left(1 + \sqrt{1-Kr^2}\right), \nonumber \\
 \Gamma^t_{\phi\phi} = {\dot{a}a}{c^2}r^2\sin^2\theta, \qquad \Gamma^{r}_{\theta\theta} = r\sqrt{1-Kr^2}\left[1-\frac{\left(1-e^2\sin^2\theta\right)^2}{1-e^2}\left(1 + \sqrt{1-Kr^2}\right)\right],\nonumber \\
\Gamma^r_{\phi\phi} = -\frac{r\sin^2\theta}{1-e^2}\left(1-Kr^2\right)\left[1-e^2\sin^2\theta + \frac{e^2\cos^2\theta}{\sqrt{1-Kr^2}}\right], \qquad \Gamma^{\phi}_{\phi r} = \Gamma^{\phi}_{r\phi} = \frac{1}{r},\nonumber \\
\Gamma^{\theta}_{\theta t} = \Gamma^{\theta}_{t\theta}= \frac{\dot{a}}{a},\qquad \Gamma^{\theta}_{rr} = - \frac{e^2\sin\theta\cos\theta\left(1- e^2\cos^2\theta\right)}{r^2\left(1-e^2\right)\left(1-Kr^2\right)}\left(1 + \sqrt{1-Kr^2}\right),\nonumber\\
\Gamma^\theta_{\theta r} = \Gamma^\theta_{r\theta} = \frac{1}{r} + \frac{e^4\cos^2\theta\sin^2\theta}{r\left(1-e^2\right)\sqrt{1-Kr^2}}\left[1+\sqrt{1-Kr^2}\right], \nonumber \\
\Gamma^{\theta}_{\theta \theta} = \frac{e^2\sin\theta\cos\theta}{1-e^2}\left(1-e^2\sin^2\theta\right)\left(1 + \sqrt{1-Kr^2}\right), \qquad \Gamma^{\phi}_{\phi\theta} = \Gamma^{\phi}_{\theta\phi} = \cot\theta,\nonumber \\
\Gamma^{\theta}_{\phi\phi} =\frac{-\sin\theta\cos\theta}{(1-e^2)}\left[1-e^2\cos^2\theta + e^2\sin^2\theta\sqrt{1-Kr^2}\right], \qquad \Gamma^{\phi}_{t\phi} = \Gamma^{\phi}_{\phi t} = \frac{\dot{a}}{a},\nonumber 
\end{eqnarray}
and the Ricci tensors and scalar:
\begin{eqnarray}
	&&R_{tt} = -3\frac{\ddot{a}}{a}, \qquad R_{tr} = R_{t\theta} = R_{t\phi} = R_{r\phi} = R_{\phi r} = 0 = R_{\phi\theta} = R_{\theta\phi}, \nonumber \\
	&&R_{rr} = \left(\ddot{a}a + 2 \dot{a}^2\right)c^2\left(1-Kr^2\right) + \frac{1}{r^2} 		+ \frac{2K}{1-Kr^2}\nonumber\\
	&&	+ 	e^2\left[\frac{1+\sqrt{1-Kr^2}}{r\left(1-e^2\right)}\left(\frac{2\cos^2\theta-\sin^2\theta	}{r\left(1-Kr^2\right)} -\sin\theta\cos\theta\right) -\left(\ddot{a}a + 2 		\dot{a}^2\right)\cos^2\theta c^2\left(1-Kr^2\right)\right]\nonumber\\
	&&+e^4 \Bigg\{\frac{\sin^4\theta\left(1+\sqrt{1-Kr^2}\right)}{r^2\left(1-e^2\right)\left(1-Kr^2\right)} + \frac{\sin^3\theta\cos\theta}{\left(1-e^2\right)\left(1-Kr^2\right)}\left(1+ \frac{1}{\sqrt{1-Kr^2}}\right) +\nonumber \\
	&&\frac{\sin^2\theta\cos^2\theta}{r^2\left(1-e^2\right)\left(1-Kr^2\right)^2}\left[-3 + 4Kr^2 + 2K^2r^4 -7 \left(1-Kr^2\right)^\frac{3}{2} + \left(K+1\right)r^2\sqrt{1-Kr^2}\right]\Bigg\}	\nonumber \\
	&&-\frac{e^6 \cos^3\theta\sin^3\theta\left(1+\sqrt{1-Kr^2}\right)}{r\left(1-e^2\right)\left(1-Kr^2\right)} + \frac{e^8\cos^3\theta\sin^4\theta\left(1+\sqrt{1-Kr^2}\right)}{r\left(1-e^2\right)^2\left(1-Kr^2\right)}\left[\sin\theta-\cos\theta\frac{1+\sqrt{1-Kr^2}}{r\sqrt{1-Kr^2}}\right]\nonumber \\
	&&R_{r\theta}=R_{\theta r} = \nonumber \\
	&& e^2\left\{\frac{\sin\theta\cos\theta}{\left(1-e^2\right)}\left[\frac{2}{3}\left(1+\sqrt{1-Kr^2}\right) -\frac{Kr}{\sqrt{1-Kr^2}} + \frac{\left(1 + \sqrt{1-Kr^2}\right)}{\left(1-e^2\right)} - \frac{\left(\ddot{a}a +\dot{a}^2r\sin\theta\cos\theta\right)}{c^2\sqrt{1-Kr^2}}\right]\right\}\nonumber \\
	&& \frac{e^4\sin\theta\cos\theta}{\left(1-e^2\right)}\Bigg\{\frac{\cos^2\theta\left(1+\sqrt{1-Kr^2}\right)}{r\left(1-Kr^2\right)}\left[2\sqrt{1-Kr^2} - 1\right]-\frac{Kr\sin^2\theta}{\sqrt{1-Kr^2}} - \frac{4}{r}\sin\theta\left(1+\sqrt{1-Kr^2}\right) \nonumber \\
	&&-\frac{3\sin^2\theta}{\left(1-e^2\right)}\left(1+\sqrt{1-Kr^2}\right)^2\Bigg\} \nonumber \\
	&& \frac{e^6\sin^3\theta\cos\theta}{\left(1-e^2\right)^2}\left(1 + \sqrt{1-Kr^2}\right)^2\left\{\frac{\cos^2\theta}{r\left(1-Kr^2\right)} + 3\sin^2\theta - e^2\sin^2\theta\left[\frac{\cos^2\theta}{r\left(1-Kr^2\right)}+ \sin^2\theta\right]\right\}\nonumber \\
	&& R_{\theta\theta} = \left(\ddot{a}a + 2\dot{a}^2 \right)r^2c^2\left(1-e^2\sin^2\theta\right) + \frac{1}{1-e^2}\left[\sqrt{1-Kr^2}\left(1-Kr^2\right) -2Kr^2\left(1+\sqrt{1-Kr^2}\right)\right]\nonumber \\
	&& + \frac{e^2}{1-e^2}\left\{\sin^2\theta\left[\left(1+ \sqrt{1-Kr^2}\right)^2 +\sqrt{1-Kr^2} -3Kr^2\left(1 + 2\sqrt{1-Kr^2}\right)\right] - \cos^2\theta\right\}\nonumber \\
	&& - \frac{e^4\sin\theta}{1-e^2}\left\{\sin^2\theta\left[\left(1+ \sqrt{1-Kr^2}\right)^2 - Kr^2\left(1+3\sqrt{1-Kr^2}\right)\right] - \cos\theta\left(1+\sqrt{1-Kr^2}\right)\left[3 + \frac{1+\sqrt{1-Kr^2}}{1-e2}\right]\right\}\nonumber \\
	&& + \frac{e^6\sin^4\theta\cos^2\theta\left(e^2\sin^2\theta-2\right)}{\left(1-e^2\right)^2}\left(1+\sqrt{1-Kr^2}\right)^2
\end{eqnarray}

==> PBH-Mass-Distribution_copy.tex <==
A convenient measure of how many primordial black holes are being produced can be given by the ratio of the energy density in primordial black holes by the total energy density
\begin{align}
	\beta
		&\equiv
								\frac{ \rho_{\rm PBH} }
								{\rho_{\rm tot}}
								\; .
								\label{eq:beta-definition}
\end{align}
Employing the standard approximation of horizon-mass collapse\footnote{Even though this assumption is wide spread in the primordial black-hole literature, it is not quite correct. A more refined treatment of the collapse exhibits a so-called critical scaling spectrum for the primordial black-hole mass distribution \cite{Choptuik:1992jv, Koike:1995jm, Gundlach:1999cu, Gundlach:2002sx}, which has been numerically verified over many orders of magnitude in density contrast in \cite{..., ..., ...}. Recently, in \cite{...}, two of us have investigated the effect of this critical scaling on the abundance of primordial black holes and found that it can in fact be very large. However, in the course of the present work, we won't take critical collapse into account in order not to defocus from the effect of non-zero ellipticity. Also, critical collapse and ellipticity are quite distinctive in nature.}, \ie~$M_{\rm PBH} \simeq M_{\rm H}$, and utilizing the Press--Schechter formalism leads to \cite{...}
\begin{align}
	\beta
		&\approx
								{\rm erfc}
								\bigg(
									\frac{ \delta_{\crm} }{ \sqrt{2\,}\.\sigma }
								\bigg)
								\notag
								\; ,
								\label{eq:beta}
\end{align}
where $\sigma$ is the root-mean square of the power spectrum subject to a given inflationary model.

In order to demonstrate the effect of ellipticity, we choose one generic model which has production of primordial black holes in a reasonable mass range. The precise nature of this model doesn't matter as {\it all} models will be effected in the same way, irrespective of the mass range in which they are peaking. We choose a particular running-mass model \cite{Stewart:1996ey, Stewart:1997wg}. In the context of primordial black-hole production, these have been intensively studied in amongst other works \cite{Drees:2011yz, Drees:2011hb, Drees:2012sz} (\cf~also~\cite{Leach:2000ea} for a discussion on constraints). The perhaps simplest realisation may be expressed through the inflationary potential
\begin{align}
	V( \phi )
		&=
								V_{0}
								+
								\frac{ 1 }{ 2 }\.m_{\phi}^{2}(\phi) \phi^{2}
								\, ,
\end{align}
with the constant $V_{0}$, and the scalar field $\phi$. There exists a plethora of embeddings of this model in various frameworks such as hybrid inflation \cite{Linde:1993cn} for instance, which lead to different specific functions $m_{\phi}( \phi )$. These yield distinct expressions for the primordial density power spectra whose variance can be recast into the general form \cite{Drees:2011hb}:
\begin{align}
	\big[ \sigma( k ) \big]^{2}
		&\simeq
								\frac{ 8 }{ 81 }\.\Pcal( k_{\star} )
								\bigg(
									\frac{ k }{ k_{\star} }
								\bigg)^{\!\! n( k ) - 1}
								\Gamma\!
								\left(
									\frac{ n_{\srm}( k ) + 3 }{ 2 }
								\right)
								\label{eq:sigma-running-mass}
								,
\end{align}
where the spectral indices $n( k )$ and $n_{\srm}( k )$ are given by 

\begin{subequations}
\begin{align}
\begin{split}
	n( k )
		&=
								n_{\srm}( k_{\star} )
								-
								\frac{ 1 }{ 2! }\.a\.\ln\!
								\bigg(
									\frac{ k }{ k_{\star} }
								\bigg)
								+
								\frac{ 1 }{ 3! }\.b\.\ln^{2}\!
								\bigg(
									\frac{ k }{ k_{\star} }
								\bigg)
								\\[1mm]
		&\phantom{=\;}
								-
								\frac{ 1 }{ 4! }\.c\.\ln^{3}\!
								\bigg(
									\frac{ k }{ k_{\star} }
								\bigg)
								+
								\ldots
								\; ,
\end{split}
								\label{eq:n-running-mass}
								\\[2mm]
\begin{split}
	n_{\srm}( k )
		&=
								n_{\srm}( k_{\star} )
								-
								a\.\ln\!
								\bigg(
									\frac{ k }{ k_{\star} }
								\bigg)
								+
								\frac{1}{2}\.b\.\ln^{2}\!
								\bigg(
									\frac{ k }{ k_{\star} }
								\bigg)
								\\[1mm]
		&\phantom{=\;}
								-
								\frac{1}{6}\.c\.\ln^{3}\!
								\bigg(
									\frac{ k }{ k_{\star} }
								\bigg)
								+
								\ldots
								\; ,
\end{split}
\end{align}
\end{subequations}
with real parameters $a$, $b$, and $c$.

Figure \ref{fig:beta-Eq} shows the ratio $\beta$ at the time of radiation-matter equality\footnote{One needs to time evolve $\beta$, being originally calculated at the time of formation, at each mass (\ie~each formation time) separately. To a good approximation the density of the primordial black holes (\wrt~the radiation background) grows like the cosmic scale factor.} for three different cases of spherical collapse (blue, solid), elliptical collapse with the parameter values of Sheth-Mo-Tormen (greed, dashed) and the one derived in this work, \cf~Eq.~\eqref{eq:delta-ec} (red, dashed).

\begin{figure}
	\centering
	\vs{-4mm}
	\includegraphics[scale=1, angle=0]{beta-Eq.pdf}
	\caption{The relative energy density $\beta^{\rm Eq}$ for the running-mass case 
		according to Eq.~\eqref{eq:sigma-running-mass}, at the time of radiation-matter equality 
		as a function of $M / M_{\odot}$.
		The blue solid curve assumes spherical collapse 
		while the dashed ones have non-zero ellipticity.
		For all graphs we choose $a = 0.011$, $b = 0.011$, $c = - 0.0010975$, as well as $\delta_{\crm} = 0.45$.
		[See the legend for specification of the parameters $\beta$ and $\gamma$.]}
	\label{fig:beta-Eq}
\end{figure}
